Integrated AHB to APB Bridge Using Raspberry Pi and Artix-7 FPGA

This project focuses on the design and implementation of an AHB to APB Bridge for efficient communication in System-on-Chip (SoC) architectures. The Advanced High-performance Bus (AHB) is used for high-speed operations, typically connecting processors and memory, while the Advanced Peripheral Bus (APB) is optimized for low-power, low-speed peripheral devices. The AHB to APB Bridge serves as an interface that converts complex, high-speed AHB transactions into simpler, single-cycle APB transactions, enabling seamless data transfer between fast components and slower peripherals. The bridge manages clock domain synchronization, transaction conversion, and flow control, ensuring compatibility between AHB's burst transfers and APB's non-pipelined protocol. Implemented in Verilog and simulated on FPGA using Xilinx Vivado, this bridge design provides a robust solution for integrating high-performance and low-power components within a single SoC. This project also evaluates the bridge's functionality and performance through testbenches covering various operational scenarios, validating its efficiency in handling diverse system requirements.

==> coverletter.tex <==



\signature{Dhandeep Challagundla\\Ignatius Bezzam\\Riadul Islam} % name for signature 
\longindentation=0pt    % needed to get closing flush left
\let\raggedleft\raggedright     % needed to get date flush left
 
\begin{letter}
{} 
\vspace{-4.5cm}
 
\opening{Dear Transactions on Very Large Scale Integration (VLSI) Reviewers:} 

\noindent We would like to thank all of you you for reviewing the paper, and the opportunity to resubmit a revised copy of the manuscript. We would like to take this opportunity to express our thanks to the reviewers for the positive feedback and helpful comments for corrections and modifications. The manuscript has been revised to address the reviewer's comments, and a separate document with responses to the reviewer's feedback has been included alongside this document.

\noindent Below is the summary of changes made to the manuscript:

\begin{enumerate}
 \setlength{\itemsep}{1pt}
 \setlength{\parskip}{0pt}
 \setlength{\parsep}{0pt}

        \item The main contributions section has been updated to provide a clearer summary of the key innovations of the work.
        \item Figure 4 has been revised to include the structure of the Sense Amplifier (SA) along with the corresponding discharge times for NAND2 and NOR2 operations.
        \item Figure 7 has been enhanced to show an example of the mapping strategy for both single-macro and three-macro implementations.
        \item The algorithm has been clarified with improved descriptions for the parts that were previously confusing, as mentioned by the reviewers.
        \item Additional clarification on the total power consumption across different macro implementations is provided for the Figure 9.
        \item A process variation analysis for the sense amplifier has been added to ensure completeness of the work.
        \item The comparison of this work with other State-of-the-Art designs has been updated.
 \end{enumerate}


   

\closing{Sincerely,}

\end{letter}


